Maximizing Alignment with Minimal Feedback: Efficiently Learning Rewards for Visuomotor Robot Policy Alignment

Visuomotor robot policies, increasingly pre-trained on large-scale datasets, promise significant advancements across robotics domains. However, aligning these policies with end-user preferences remains a challenge, particularly when the preferences are hard to specify. While reinforcement learning from human feedback (RLHF) has become the predominant mechanism for alignment in non-embodied domains like large language models, it has not seen the same success in aligning visuomotor policies due to the prohibitive amount of human feedback required to learn visual reward functions. To address this limitation, we propose Representation-Aligned Preference-based Learning (RAPL), an observation-only method for learning visual rewards from significantly less human preference feedback. Unlike traditional RLHF, RAPL focuses human feedback on fine-tuning pre-trained vision encoders to align with the end-user's visual representation and then constructs a dense visual reward via feature matching in this aligned representation space. We first validate RAPL through simulation experiments in the X-Magical benchmark and Franka Panda robotic manipulation, demonstrating that it can learn rewards aligned with human preferences, more efficiently uses preference data, and generalizes across robot embodiments. Finally, our hardware experiments align pre-trained Diffusion Policies for three object manipulation tasks. We find that RAPL can fine-tune these policies with 5x less real human preference data, taking the first step towards minimizing human feedback while maximizing visuomotor robot policy alignment.

==> sections/intro.tex <==

\section{Introduction}

Recent efforts in open-source datasets of expert demonstrations \cite{ettinger2021large,padalkar2023open} have greatly accelerated the development of robotics foundation models across diverse domains, including autonomous driving \citep{seff2023motionlm, philion2024trajeglish}, robot manipulation \citep{brohan2023rt}, and humanoid locomotion \citep{radosavovic2024humanoid}. 
%
While these large-scale datasets enable us to leverage high-capacity models and scaling laws, pushing the boundaries of generalization, they also restrict the robot learning paradigm to imitation learning due to the absence of reward labels and compatible simulation environments.
Consequently, these models often lack an in-depth understanding of human preferences, resulting in undesirable behaviors at best and safety hazards at worst \cite{lu2023imitation}. 


When operating in service of people, robots need to optimize their behaviors to align with end-user preferences. Drawing from advances in Large Language Model research, we argue that robotics foundation models will similarly require an alignment phase, where the initial robot policy is fine-tuned to better meet the preferences and expectations of end-users.
% 
Fundamentally, generative model alignment depends on the end-user’s reward function—their internal mapping from a model’s outputs to a scalar measure of ``goodness"—as a signal for guidance. Since we don’t have direct access to this function, we typically rely on human feedback like demonstrations, preference rankings, binary labels, corrections, etc., to either learn an explicit reward model for fine-tuning the model via reinforcement learning \cite{ouyang2022training} or directly fine-tune the model using contrastive methods based on preference rankings of robot policy rollouts \cite{rafailov2024direct}. 

Unfortunately, for robotics foundation models, gathering sufficient feedback from end-users—whether through demonstrations or rankings—is prohibitively costly. Unlike writing text, where users are naturally familiar with the medium, many everyday users lack experience with robotic systems, making it challenging for them to teleoperate robots effectively to provide optimal demonstrations for policy refinement. Although preference rankings reduce the need for users to be expert demonstrators, they still impose a substantial time cost, especially for end-to-end behavior models that process raw images. Users would need to review thousands of robot rollouts to provide enough annotations to directly align these models, making the process highly time-intensive.


In this work, we propose an alignment approach that enables learning \textbf{\textit{more accurate visual rewards}} with \textbf{\textit{less human feedback}}, specifically designed to align robot behavior generation models effectively.



Our approach builds upon the insights from foundational work on inverse reinforcement learning \cite{abbeel2004apprenticeship, ziebart2008maximum}, which advocates for using feature distribution matching to assess the alignment between robot behaviors induced by a recovered reward function and the end-user's demonstrations. In other words, if the feature distribution of robot behaviors closely matches that of the end-user’s demonstrations, the recovered reward function is considered better aligned with the end-user’s true reward function. 
%
This insight was initially developed for hand-designed features operating on low-dimensional state representations \cite{finn2016guided,levine2011nonlinear}. Nevertheless, revisiting this idea in the era of robotics foundation models (that operate on high-dimensional observations) 
reveals precisely where to best allocate our limited human feedback budget: 

\textit{Our key idea is that we should focus our human feedback on our aligning vision encoders, learning specifically what visual features ``matter" to the end-user! }

\noindent
From there, the robot can rely on visual embedding distribution matching to produce either explicit reward values or implicit preference rankings, effectively aligning its behavior generation model with much less human feedback than prior methods.

 

In Section~\ref{sec:RAPL method}, we first formalize the visual representation alignment problem for robotics as a metric learning problem in the human's representation space. 
We then propose \textbf{R}epresentation-\textbf{A}ligned \textbf{P}reference-based \textbf{L}earning (\textbf{RAPL}), a tractable video-only method for solving the alignment problem and learning visual robot rewards via optimal transport. 




Empirically, in Section~\ref{sec:RAPL-result}, we first demonstrate that RAPL learns visual rewards that consistently align more closely with the ground truth rewards and enables a more data-efficient and effective RLHF paradigm for aligning visual-motor robot policies. Across experiments in the X-Magical benchmark and in robotic manipulation, we find that RAPL’s reward consistently aligns more closely with the ground truth reward with high sample efficiency, generates more preferred robot behaviors, and shows strong zero-shot generalization when the visual representation is learned on a different embodiment than the robot’s.


Finally, in Section~\ref{sec:DPO-result}, we demonstrate how RAPL enables alignment of robotics foundation models in the real world without requiring a simulator, using direct preference optimization (DPO) with synthetic preference rankings. We show that RAPL significantly reduces the need for real human preference rankings, allowing the reference robot behavior model to align more efficiently with human preferences.


==> sections/visual_reward_experiment_results.tex <==
\section{Experiment Result-Visual Reward Learning}
\label{sec:result-reward-learning}

In this section, we design a series of experiments to evaluate RAPL’s effectiveness in learning visual rewards.

\subsection{Experimental Design }

% We first detail the experimental design and then present our simulation environments and results. 
% want to study three questions: 1) \textit{Does RAPL's visual reward yield robot policies that are aligned with end-user preferences?} and 2) \textit{How much does an aligned visual representation matter for generating preferred robot behaviors?}, and 3) \textit{What sample complexity gains does our method achieve compared to direct reward prediction?} 

% \subsection{Experimental Design}

\textbf{Preference Dataset: $\tilde{S}_{\reph}$.} While the ultimate test is learning from real end-user feedback, in this section, we first use a simulated human model, which allows us to easily ablate the size of the preference dataset, and gives us privileged access to $\rewh$ for direct comparison.
In all environments, the simulated human constructs the preference dataset $\tilde{S}_{\reph}$ by sampling triplets of videos uniformly at random from the set\footnote{To minimize the bias of this set on representation learning, we construct $\tilde{\Xi}$ such that the reward distribution of this set under  $\rewh$, is approximately uniform. Future work should investigate the impact of this set further, e.g., \citep{sadigh2017active}.} of video observations $\tilde{\Xi} \subset \Xi$, and then ranking them with their reward $\rewh$ as in  \autoref{eq:representation_alignment_loss}. 

\noindent
\textbf{Independent \& Dependent Measures.} Throughout our experiments we vary the \textit{visual reward signal} used for robot policy optimization. %and the \textit{preference dataset size} used for representation learning. 
The reward signal includes varying the visual representation, how the reward is trained, etc. 
We measure the Spearman’s correlation to evaluate the relationship between the learned visual reward and the end-user’s ground-truth reward. 
% The success rate is the 



\subsection{Results: X-Magical}
\label{subsec:reward-xmagical}

We first experiment in the toy X-Magical environment \citep{zakka2022xirl}, and then move to the realistic IsaacGym simulator. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/sim_environments_2.png}
    %\vspace{-0.7cm}
  \caption{X-Magical \& IsaacGym tasks.}
  %\vspace{-0.5cm}
  \label{fig:x-magical-env}
\end{figure}

\noindent
\textbf{Tasks.}  We design two tasks inspired by kitchen countertop cleaning. The robot always has to push objects to a goal region (e.g., trash can), shown in pink at the top of the scene in \autoref{fig:x-magical-env}. In the \textbf{avoiding} task, the end-user prefers that the robot and objects never enter an \textit{off-limits zone} during pushing (blue box in left \autoref{fig:x-magical-env}).
% where the robot needs to push the object (red square) towards a static goal region (light red region) without entering a disfavored region (light blue region). 
In the \textbf{grouping} task, the end-user prefers that objects are always pushed \textit{efficiently together} (instead of one-at-a-time) towards the goal region (center, \autoref{fig:x-magical-env}).


\noindent
\textbf{Privileged State \& Reward.}
For \textbf{avoiding}, the true state $s$ is 7D: planar robot position ($p_\robot \in \mathbb{R}^2$) and orientation ($\theta_\mathrm{R}$),  planar position of the object ($p_{\mathrm{obj}}\in \mathbb{R}^2$), distance between goal region and object, ($d_{\mathrm{obj2goal}}$), and distance between the off-limits zone and the object ($d_{\mathrm{obs2obj}}$). The human's reward is: $\rewh_{\mathrm{avoid}}(s) = - d_{\mathrm{goal2obj}} - 2\cdot \mathbb{I}(d_{\mathrm{obs2obj}} < d_{\mathrm{safety}})$, where $d_{\mathrm{safety}}$ is a safety distance and $\mathbb{I}$ is an indicator function giving $1$ when the condition is true.
For \textbf{grouping}, the state is 9D: $s := (p_\robot, \theta_\robot$, $p_{\mathrm{obj^1}}, p_{\mathrm{obj^2}}, d_{\mathrm{goal2obj^1}}$, $d_{\mathrm{goal2obj^2}})$. The human's reward is: $\rewh_{\mathrm{group}}(s) = - \max(d_{\mathrm{goal2obj^1}}, d_{\mathrm{goal2obj^2}}) - ||p_{\mathrm{obj^1}} - p_{\mathrm{obj^2}}||_2$.

\noindent
\textbf{Baselines.} We compare our visual reward, \rapl, against (1) \gt, an oracle policy obtained under $\rewh$, (2) \rlhf, which is vanilla preference-based reward learning \citep{christiano2017deep, brown2019extrapolating} that directly maps an image observation to a scalar reward, and (3) \tcc \citep{zakka2022xirl,kumar2023graph} which finetunes a pre-trained encoder via temporal cycle consistency constraints using 500 task demonstrations and then uses L2 distance between the current image embedding and the goal image embedding as reward. We use the same preference dataset with $150$ triplets for training RLHF and RAPL. 

% =========== XMAGICAL ============= %
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figs/xmagical_indomain_reward_new.pdf}
    \vspace{-1em}
    \caption{\textbf{X-Magical.} (left \& right) examples of preferred and disliked videos for each task. (center) reward associated with each video under each method. RAPL's predicted reward follows the GT pattern: low reward when the behavior are disliked and high reward when the behavior are preferred. RLHF and TCC assign high reward to disliked behavior (e.g., (D)). }
    \vspace{-1em}
    \label{fig:xmagical_indomain_reward}
\end{figure*}


\noindent
\textbf{Visual model backbone.} We use the same setup as in \citep{zakka2022xirl} with the ResNet-18 visual backbone \citep{he2016deep} pre-trained on ImageNet. The original classification head is replaced with a linear layer that outputs a $32$-dimensional vector as our embedding space, $\Phi_\robot := \mathbb{R}^{32}$. The TCC representation model is trained with 500 demonstrations using the code from \citep{zakka2022xirl}. Both RAPL and RLHF only fine-tune the last linear layer. All representation models are frozen during policy learning.

\noindent
\textbf{Hypothesis}. \textit{\rapl is better at capturing preferences \textit{beyond} task progress compared to direct reward prediction \rlhf or \tcc visual reward, yielding higher success rate.} 



\noindent
\textbf{Results.} 
Figure~\ref{fig:xmagical_indomain_reward} shows the rewards over time for three example video observations in the \textbf{avoid} (left) and \textbf{group} task (right). Each video is marked as preferred by the end-user's ground-truth reward or disliked. 
% \rapl rewards withe the baseline visual rewards and the \gt rewards for the avoiding task (left) and the grouping task (right). 
Across all examples, \rapl's rewards are highly correlated with the \gt rewards: when the behavior in the video is disliked, then reward is low; when the behavior is preferred, then the reward is increasing. \tcc's reward is correlated with the robot making spatial progress (i.e., plot (E) and (F) where observations get closer to looking like the goal image), but it incorrectly predicts high reward when the robot makes spatial progress but violates the human's preference ((C) and (D) in \autoref{fig:xmagical_indomain_reward}). \rlhf performs comparably to \rapl, with slight suboptimality in scenarios (C) and (D). \tr{Refer to the table}



\subsubsection{Robot Manipulation}
\label{subsec:in-domain-manipulation}

\begin{center}
\justifying
In the X-Magical toy environment, RAPL outperformed progress-based visual rewards, but direct preference-based reward prediction was a competitive baseline. Moving to the more realistic robot manipulation environment, we want to 1) disentangle the benefit of our fine-tuned representation from the optimal transport reward structure, and 
% is the benefit of \rapl attributed by optimal transport only?
2) understand if our method still outperforms direct reward prediction in a more complex environment?
\end{center}


% ======== IN-DOMAIN: MANIPULATION  REWARD ======= %
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figs/franka_OT_rew_indomain_new.pdf}
    \caption{\textbf{Manipulation. }   
    (center) Expert, preferred, and disliked video demo.
    (left) reward associated with each video under each method. RAPL's predicted reward follows the GT pattern. RLHF assigns high reward to disliked behavior.
    % Across both types of demos, \rapl matches the same reward trends as \gt, while other methods struggle to disambiguate. 
    (right) OT coupling for each representation. Columns are embedded frames of expert demo. Rows of top matrices are embedded frames of preferred demo; rows of bottom matrices are embedded frames of disliked demo. Peaks exactly along the diagonal indicate that the frames of the two videos are aligned in the latent space; uniform values in the matrix indicate that the two videos cannot be aligned (i.e., all frames are equally ``similar’’ to the next). RAPL matches this structure: diagonal peaks for expert-and-preferred and uniform for expert-and-disliked, while baselines show diffused values no matter the videos being compared.}
    \label{fig:franka_OT_rew_indomain}
    \vspace{-1em}
\end{figure*}


\noindent
\textbf{Task.} We design a robot manipulation task in the IsaacGym physics simulator \citep{makoviychuk2021isaac}. We replicate the tabletop \textbf{grouping} scenario, where a Franka robot arm needs to learn that the end-user prefers objects be pushed \textit{efficiently together} (instead of one-at-a-time) to the goal region (light blue region in right of \autoref{fig:x-magical-env}). 

\noindent
\textbf{Privileged State \& Reward.}
The state $s$ is 18D: robot proprioception ($\theta_{\mathrm{joints}}\in \mathbb{R}^{10}$), 3D object positions
($p_{\mathrm{obj^{1,2}}}$), and object distances to goal ($d_{\mathrm{goal2obj^{1,2}}}$). The \textbf{grouping} reward is identical as in Section~\ref{subsec:in-domain-xmagical}. 

\noindent
\textbf{Baselines.} In addition to comparing \rapl against (1) \gt and (2) \rlhf, we ablate the \textit{representation model} but control the \textit{visual reward structure}. We consider five additional baselines that all use optimal transport-based reward but operate on different representations: (3) \mvpot which learns image representation via masked visual pre-training; \prb{(4) \mvpotfinetune, which fine-tunes MVP representation  using images from the task environment; (5) \rtm, which is an off-the-shelf ResNet-18 encoder \citep{nair2022r3m} pre-trained on the Ego4D data set \citep{grauman2022ego4d} via a learning objective that combines time contrastive learning, video-language alignment, and a sparsity penalty; (6): \imagenet, which is a ResNet-18 encoder pre-trained on ImageNet;} (7) \tccot \citep{dadashi2020primal} which embeds images via the TCC representation trained with 500 task demonstrations. We use the same preference dataset with $150$ triplets for training RLHF and RAPL.


\noindent
\textbf{Visual model backbone.} All methods except MVP-OT and Fine-Tuned-MVP-OT share the same ResNet-18 visual backbone and have the same training setting as the one in the X-Magical experiment. MVP-OT and Fine-Tuned-MVP-OT use a off-the-shelf visual transformer \citep{xiao2022masked} pre-trained on the Ego4D data set \citep{grauman2022ego4d}. All representation models are frozen during policy learning.

\noindent
\textbf{Hypotheses}. \textbf{H1:} \textit{\rapl's higher success rate is driven by its aligned visual representation}. \textbf{H2:} \textit{\rapl outperforms \rlhf with lower amounts of human preference queries}.




% ======== IN-DOMAIN: MANIPULATION POLICY ======= %

\begin{figure}
    %\vspace{-0.5cm}
    \includegraphics[width=0.45\textwidth]{figs/franka_success_v_reward_all_baselines.pdf}
    %\vspace{-0.8cm}
  \caption{\textbf{Manipulation.} Success rate during robot policy learning for each visual reward. }
  %\vspace{-0.2cm}
  \label{fig:franka_success_v_reward}
\end{figure}


\noindent
\textbf{Results: Reward prediction \& policy learning.} 
In the center of Figure~\ref{fig:franka_OT_rew_indomain} we show three video demos: an expert video demonstration, a preferred video, and a disliked video. 
On the right of Figure~\ref{fig:franka_OT_rew_indomain}, we visualize the optimal transport plan comparing the expert video to the disliked and preferred videos under each visual representation, $\phi_{\rapl}$, $\phi_{\tccot}$, $\phi_{\mvpot}$. Intuitively, peaks exactly along the diagonal indicate that the frames of the two videos are aligned in the latent space; uniform values in the matrix indicate that the two videos cannot be aligned (i.e., all frames are equally ``similar’’ to the next).
\rapl's representation induces precisely this structure: diagonal peaks when comparing two preferred videos and uniform when comparing a preferred and disliked video. 
% The transport plan has peak values along the diagonal when transporting the preferred trajectory's empirical aligned embedding distribution to that of the expert trajectory, indicating high alignment between the two, and has evenly spread values when transporting disliked trajectory's empirical aligned embedding distribution to the expert's, indicating poor alignment between the two. 
Interestingly, we see diffused peak regions in all transport plans under both \tccot and \mvpot representations, indicating their representations struggle to align preferred behaviors and disentangle disliked behaviors.
This is substantiated by the left of Figure~\ref{fig:franka_OT_rew_indomain}, which shows the learned reward over time of preferred video and disliked video. Across all examples, \rapl rewards are highly correlated to \gt rewards while baselines struggle to disambiguate, supporting \textbf{H1}.

Figure~\ref{fig:franka_success_v_reward} shows the policy evaluation history during RL training with each reward function. We see \rapl performs comparably to \gt (succ. rate: $\approx 70\%)$ while all baselines struggle to achieve a success rate of more than $\approx 10\%$ with the same number of epochs.


% ======== MANIPULATION  Attention MAP ======= %

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/attention_map.png}
    \caption{\textbf{Manipulation: Attention Map.} Visualization of attention map for RLHF-150 demos, RLHF-300 demos, and RAPL with 150 demos for both Franka and Kuka (cross-embodiment) images. Each entry of the figure shows two image snapshots from the relevant demonstration set with the attention map overlaid. Bright yellow areas indicate image patches that contribute most to the final embedding; darker purple patches indicate less contribution. $\phi_{RLHF-150}$ is biased towards paying attention to irrelevant areas that can induce spurious correlations; in contrast RAPL learns to focus on the task-relevant objects and the goal region. $\phi_{RLHF-300}$'s attention is slightly shifted to objects while still pays high attention to the robot embodiment.}
    \label{fig:attention_map}
\end{figure*}


\noindent
\textbf{Results: Sample complexity comparison between of \rapl and \rlhf.}
%
It's surprising that \rlhf fails in a more realistic environment since its objective is similar to ours, but without explicitly considering representation alignment.
%
To further investigate this, we apply a linear probe on the final embedding and visualize the image heatmap of what \rapl's (our representation model trained with 150 training samples), \rlhf-150's (\rlhf trained with 150 samples), and \rlhf-300's (\rlhf trained with 300 samples samples) final embedding pays attention to in Figure~\ref{fig:attention_map} (detailed explains about the linear probe are in the Appendix). 
We see that $\phi_{RAPL}$ learns to focus on the objects, the contact region, and the goal region while paying less attention to the robot arm;
$\phi_{RLHF-150}$ is biased towards
paying attention to irrelevant areas
that can induce spurious correlations (such as the robot arm and background area);
$\phi_{RLHF-300}$'s attention is slightly shifted to objects while still pays high attention to the robot embodiment.
%
When deploying $\phi_{RLHF-300}$ in Franka manipulation policy learning (Figure~\ref{fig:rlhf_double_datasize}), we observe that policy performance is slightly improved, indicating that with more feedback data, preference-based reward prediction could yield an aligned policy. Nevertheless, \rapl outperforms \rlhf by $75\%$ with $50\%$ less training data, supporting \textbf{H2}. 
  




While all the RAPL results above used 150 preference queries to train the representation, we also train a visual representation with 100, 50, and 25 preference queries.  Figure~\ref{fig:rapl_sample_size_exp} shows the success rate of the robot manipulation policy for each version of RAPL. 
We note that \rapl achieves a 45\% success rate even when trained on only 25 preference queries.




\begin{figure}
    %\vspace{-0.0cm} 
    \includegraphics[width=0.4\textwidth]{figs/franka_rlhf_double_data.png}
    %\vspace{-0.5cm}
    \caption{\textbf{Manipulation.} \rapl outperforms \rlhf by $75\%$ with $50\%$ less training data.}
    \label{fig:rlhf_double_datasize}
    %\vspace{-0.5cm}
\end{figure}

\begin{figure}
    %\vspace{-0.5cm} 
    \centering
    \includegraphics[width=0.35\textwidth]{figs/OT_datasize_exp.png}
    %\vspace{-0.6cm}
    \caption{\textbf{Manipulation.} \rapl sample efficiency analysis. RAPL can achieve $\approx$ 45\% success rate with only 25 preference queries.}
    \label{fig:rapl_sample_size_exp}
    %\vspace{-0.5cm}
\end{figure}

\subsubsection{Additional Complex Manipulation Task with Visual Distractors}
\label{subsec: multi object push}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figs/fanka_push_multi_objs.pdf}
    \caption{\rb{\textbf{Clutter task: Complex robot manipulation with visual distractors}. (left) Visualization of preferences. Green (preferred behavior): the Franka arm grasps the green rectangular prism and uses that to push the red rectangular prism to the goal region. Red (negative behavior): the Franka arm fails to grasp the rectangular prism. (right) Policy training results for our method and additional baselines.}}
    \vspace{-0.3cm}
    \label{fig:franka_multi}
\end{figure*}



\begin{center}
\justifying
Finally, we consider a more complex robot manipulation task---named \textbf{clutter} in the text and charts---to further validate \rapl's ability to disentangle visual features that underlie an end-user's preferences. 
We increase the difficulty of the the robot manipulation environment described in Section~\ref{subsec:in-domain-manipulation} by adding visual distractors that are irrelevant to the human's preferences (left figure in Figure~\ref{fig:franka_multi}). 
The environment has multiple objects on the table of various colors---red, green, and goal-region-blue---and some of the objects are cubes while others are rectangular prisms.
The Franka robot arm needs to learn that the end-user prefers to push the \textit{rectangular} objects (instead of the cubes) \textit{efficiently together} (instead of one-at-a-time) to the goal region. 
% Here, the color of the objects is a visual distractor and is irrelevant to the person's preference. 
\end{center}

\noindent
\textbf{Task Complexity \& Feature Entanglement.} Compared to the manipulation task described in Section~\ref{subsec:in-domain-manipulation}, the Franka arm needs to learn representations that can disentangle both semantic preference (grouping) and low-level preference (shape) from RGB images under visual distractors (object color). In addition, the Franka arm needs to learn to \textit{grasp} the rectangular prism first and use that to push the second rectangular prism, as it is difficult to directly push the rectangular prism stably using the robot finger gripper, thus increasing the task difficulty.

\noindent
\textbf{Privileged State \& Reward.}
The state $s$ is 34D: robot proprioception ($\theta_{\mathrm{joints}}\in \mathbb{R}^{10}$), 3D object positions
($p_{\mathrm{obj_{rect}^{1,2}}}, p_{\mathrm{obj_{cube}^{1,\dots,4}}}$), and object distances to goal ($d_{\mathrm{goal2obj_{rect}^{1,2}}}, d_{\mathrm{goal2obj_{cube}^{1,\dots,4}}}$). The simulated human's reward is:
\begin{align*}
    \rewh_{\mathrm{group}}(s) &= - \max(d_{\mathrm{goal2obj^{rect,1}}}, d_{\mathrm{goal2obj^{rect,2}}}) \\ & \quad\quad - ||p_{\mathrm{obj_{rect}^{1}}} - p_{\mathrm{obj_{rect}^{2}}}||_2 \\ &\quad\quad - 0.1 \sum_{i=1}^{4} ||p_{\mathrm{obj_{cube}^{i}}} - p_{\mathrm{obj_{cube}^{i, init}}}||_2.
\end{align*}




% \textbf{Baselines.} In addition to comparing \rapl against (1) \gt and (2) \rlhf, we ablate the \textit{representation model} but control the \textit{visual reward structure}. We consider four additional baselines that all use an optimal transport-based reward but operate on different representations: (3): \mvpot which is a off-the-shelf visual transformer \citep{xiao2022masked} pre-trained on the Ego4D data set \citep{grauman2022ego4d} via masked visual pre-training; (4): \mvpotfinetune which fine-tunes \mvpot using images from the task environment via LoRA \citep{hu2021lora}; (5): \rtm which is an off-the-shelf ResNet-18 encoder \citep{nair2022r3m} pre-trained on the Ego4D data set \citep{grauman2022ego4d} via a learning objective that combines time contrastive learning, video-language alignment, and a sparsity penalty; (6): \imagenet which is an off-the-shelf ResNet-18 encoder pre-trined on ImageNet. We use the same preference dataset with $150$ triplets for training RLHF and RAPL. 

\noindent
\textbf{Results.} The right plot in Figure~\ref{fig:franka_multi} shows the policy evaluation history during RL training with each reward function. We see \rapl performs comparably to \gt (succ. rate: $\approx 65\%)$ while all baselines struggle to achieve a success rate of more than $\approx 10\%$ with the same number of epochs.




\subsubsection{Spearman’s correlation between GT and learned visual rewards}
\begin{center}
\justifying
\prb{We conducted a quantitative analysis to investigate the relationship between the learned visual reward and the end-user’s ground-truth reward. For the robot manipulation tasks described in Section~\ref{subsec:in-domain-manipulation} (Franka Group), Section~\ref{sec:cross-domain-results} (Kuka Group), and Section~\ref{subsec: multi object push} (Franka Clutter), we computed the average Spearman’s correlation coefficient between the ground-truth reward trajectory and any other approach's reward trajectory across 100 video trajectories. We found that \rapl's learned visual reward shows the strongest correlation to the \gt reward compared to baselines.
\end{center}

\renewcommand{\arraystretch}{1.5}
\begin{table}[h!]
    \centering
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{| p{0.7in} | c | c | c | }
    \hline
       & \multicolumn{3}{|c|}{ \textbf{Spearman's Correlation} } \\ \hline 
         & \textbf{Franka Group} (Sec.~\ref{subsec:in-domain-manipulation}) & \textbf{Kuka Group} (Sec.~\ref{sec:cross-domain-results}) & \textbf{Franka Clutter} (Sec.~\ref{subsec:in-domain-manipulation}) \\ \hline
        \rapl & \textbf{0.59} &  \textbf{0.47} & \textbf{0.61}\\ \hline
        \rlhf & 0.38 &  0.31 & 0.26\\ \hline
        \mvpot &  -0.1&  0.02 & 0.08\\ \hline
        \mvpotfinetuneabbrev &  0.19&  0.02& 0.11 \\ \hline
        \imagenetabbrev &  -0.09 &  0.12 & -0.02\\\hline
        \rtm & 0.03 &  -0.14 &  -0.17 \\ \hline
    \end{tabular}
    }
    \caption{\rb{Spearman's rank correlation coefficient between the \gt reward and each learned reward.}}
    \label{table:Spearman}
\end{table}





\subsection{Results: Zero-Shot Generalization Across Embodiments}
\label{sec:cross-domain-results}

So far, the preference feedback used for aligning the visual representation was given on videos $\obstraj \in \tilde{\Xi}$ generated on the same embodiment as that of the robot. 
However, in reality, the human could give preference feedback on videos of a \textit{different} embodiment than the specific robot's.
% However, in reality, the easiest interface for soliciting preferences could be for the human to directly \textit{show themselves} performing the task in desired and less desired ways. 
% Thus, the preference dataset $\tilde{S}_\human$ used for aligning the representation will be generated on a \textit{different} embodiment than the robot's. 
We investigate if our approach can \textit{generalize} to changes in the embodiment between the preference dataset $\tilde{S}_\human$ and the robot policy optimization. 

% ========== XMAGICAL: CROSS EMBODIMENT =========== %
\begin{figure*}[h]
    \centering
    \vspace{-0.5cm}
    \includegraphics[width=0.85\textwidth]{figs/xmagical_crossdomain_policy.pdf}
    \vspace{-1.5em}
    \caption{\textbf{Cross-Embodiment: X-Magical.} Policy evaluation success rate during policy learning. Colored lines are the mean and variance of the evaluation success rate. RAPL achieves a comparable success rate compared to GT with high learning efficiency, and outperforms RLHF and TCC.}
    \vspace{-1em}
    \label{fig:xmagical_crossdomain_policy}
\end{figure*}

\noindent
\textbf{Tasks \& Baselines.} We use the same setup for each environment as in Section~\ref{sec:in-domain-results}.

\noindent
\textbf{Cross-Domain Agents.} In X-Magical, reward functions are always trained on the \textit{short stick} agent, but the learning agent is a \textit{gripper} in \textbf{avoid} and a \textit{medium stick} agent in \textbf{grouping} task. In robot manipulation we train RAPL and RLHF on videos of the \textit{Franka} robot, but deploy the rewards on the \textit{Kuka} robot.

\noindent
\textbf{Hypothesis.} \textit{\rapl enables zero-shot cross-embodiment generalization of the visual reward compared to other visual rewards.}


% the world may be different when the human and the robot generate data because the two agents do not share the same embodiment. For example, instead of teleoperating the robot, the human may want to show how to do the task on their own. The robot learns its representation and visual reward from this dataset that is generated on the human's embodiment, but then has to optimize this visual reward \textit{on its own} embodiment. 

% \tr{Maybe just highlighting the x-magical and manipulation RL results together here, and put the reward vis in the appendix?}
% \abnote{Yes, I think thats a great idea.}



\noindent
\textbf{Results.} 
Figure~\ref{fig:xmagical_crossdomain_policy} and  Figure~\ref{fig:kuka_success_v_reward} show the policy evaluation histories during RL training with each reward function in the cross-embodiment X-Magical environment and the manipulation environment. We see that in all cross-embodiment scenarios, \rapl achieves a comparable success rate compared to \gt and significantly outperforms baselines which struggle to achieve more than zero success rate, supporting \textbf{H1}. See more results in App. \ref{app:cross-domain-results}, which demonstrate that RAPL’s rewards are highly correlated with the \gt rewards even when deployed on a cross-embodiment robot.


% ========== Manipulation: CROSS EMBODIMENT =========== %
\begin{figure}
    %\vspace{-0.5cm}
    \includegraphics[width=0.45\textwidth]{figs/kuka_success_v_reward_all_baselines.pdf}
    %\vspace{-0.5cm}
  \caption{\textbf{Cross-Embodiment: Manipulation.} Colored lines are the mean and variance of the success rate during policy learning.}
  %\vspace{-0.2cm}
  \label{fig:kuka_success_v_reward}
\end{figure}



We note an interesting finding in the X-Magical grouping task when the representation is trained on videos of the \textit{short stick} agent, but the learning agent is the \textit{medium stick} agent. %(see Figure~\ref{fig:xmagical_crossdomain_reward} in Appendix). 
Because the \textit{short stick} agent is so small, it has a harder time keeping the objects grouped together; in-domain results from Section~\ref{sec:in-domain-results} show a success rate of $\approx$ 60\% (see Figure~\ref{fig:xmagical_indomain_policy}). 
In theory, with a well-specified reward, the task success rate should \textbf{increase} when the \textit{medium stick} agent does the task, since it is better suited to push objects together. 
Interestingly, when the \textit{short stick} visual representation is transferred zero-shot to the \textit{medium stick}, we see precisely this: \rapl's task success rate \textbf{improves} by 20\% under cross-embodiment transfer (succ. rate $\approx$ 80\%). 
% The finding that our visual representation can be learned from videos of an embodiment that struggles to do object grouping effectively, but then can be zero-shot transferred to an embodiment that can do the task easily 
This finding indicates that RAPL can learn task-relevant features that can guide correct task execution even on a new embodiment. 


